Curvature Prior for MRF-based Segmentation and Shape Inpainting

Most image labeling problems such as segmentation and image reconstruction are fundamentally ill-posed and suffer from ambiguities and noise. Higher order image priors encode high level structural dependencies between pixels and are key to overcoming these problems. However, these priors in general lead to computationally intractable models. This paper addresses the problem of discovering compact representations of higher order priors which allow efficient inference. We propose a framework for solving this problem which uses a recently proposed representation of higher order functions where they are encoded as lower envelopes of linear functions. Maximum a Posterior inference on our learned models reduces to minimizing a pairwise function of discrete variables, which can be done approximately using standard methods. Although this is a primarily theoretical paper, we also demonstrate the practical effectiveness of our framework on the problem of learning a shape prior for image segmentation and reconstruction. We show that our framework can learn a compact representation that approximates a prior that encourages low curvature shapes. We evaluate the approximation accuracy, discuss properties of the trained model, and show various results for shape inpainting and image segmentation.

==> tex/discussion_old.tex <==
\section{Discussion}\label{discussion}
\begin{itemize}
\item thin lines can be handled by adding specific patterns
\item bottom-up cues -- data-driven selection of possible patterns
\item refine patterns during iterations or use as initialization for other methods
\item Optimization: ambiguous min-marginals issue, optimization ``improve'' method: (block-)ICM or restricted problem, factor-graph BP = BP, parallelization.
\item our method could be used as initialization of continuouse method
\end{itemize}

==> tex/discussion_old1.tex <==
\section{Discussion}\label{discussion}

%Let us point some limitations and possibilities.
Several remarks about the model. The current model does not allow very thin objects, as patterns assume the shape is at least 4 pixels thick. However, this would be automatically handled, if we sampled such shapes during the training.

Solutions we construct based on TRW-S tree min-marginals could be very spiky on the pixel level: this is due to independent choice of labels for ambiguous tree min-marginals. However, sequential fixation strategy~\cite{Kolmogorov-06-convergent-pami} introduces directional dependence and can create strange artifacts in the inpainting problems. We think we can get better results by a discrete local search method, such as (block-)ICM, started from our solution. On the other hand, our solution could be used as a good starting point for a continuous method.


We see some inconsistency in that we formulate and learn the model in discrete variables, perform optimization in the relaxation, but unlike~\cite{Schoenemann09} cannot obtain a globally optimal discrete solution. Indeed, we haven't observed 0 integrality gap even for simple test problems solved with primal LP solver. This suggest that we might want to train the model such that the {\em relaxation} provides the best representation of a shape and approximation of the cost.

%
%
%It turned out that the relaxed primal labeling, when we could compute it,
%
%Optimization is difficult. Some of the discrete solutions we obtained from TRW-S tree min-marginals are spiky on the pixel level. When min-marginals are ambiguous, the solution is up to numerical
%
%Optimization: ambiguous min-marginals issue, optimization ``improve'' method: (block-)ICM or restricted problem, factor-graph BP = BP, parallelization.

%Optimization with TRW-S is computationally intensive. We see several possibilities to speed it up. The model could be put into coarse-to-fine framework, in terms of both spatial resolution and number of patterns. %It could also benefit from bottom-up cues such as candidate edges.

%\par

%\begin{itemize}
%\item thin lines can be handled by adding specific patterns
%\item bottom-up cues -- data-driven selection of possible patterns
%\item refine patterns during iterations or use as initialization for other methods
%\item Optimization: ambiguous min-marginals issue, optimization ``improve'' method: (block-)ICM or restricted problem, factor-graph BP = BP, parallelization.
%\item our method could be used as initialization of continuouse method
%\end{itemize}

==> tex/experiments_PS.tex <==
\section{Experiments}\label{experiments}
We now describe the results of our experiments.
%
{\bf Cost approximation} To learn a curvature model with 96 patterns
of size $K=8$, we sampled $N=10000$ random quadratic curves passing
close to the center in a $K{\times}K$ pixel patch (see
fig.~\ref{fig:pointwise}). We split them into $32$ orientations and
$3$ curvature intervals to learn the initial pattern based curvature
model. Fig.~\ref{fig:alg1_progress} shows the error of the estimate
measured by~\eqref{pointwise_approx} and progress of Alg.1., while
Fig.~\ref{fig:pointwise} shows individual approximations of
individual test quadratic curves.
\par
It can be seen from Fig.~\ref{fig:pointwise} that the pointwise
approximation is not accurate. However, this problem should be
overcome when the costs are summed up along the boundary as they
will give a good approximation on average. For this purpose, we
sampled larger shapes for which we can compute true total cost
exactly and then compared them to those produced by our model.
Fig.~\ref{fig:total_cost}(a,b) shows this experiment for two classes
of shapes: (1) Circular shapes of size $100{\times}100$ with random
radius (uniformly sampled in [5 50] pixels) and subpixel shift (
Fig.~\ref{fig:total_cost}a). (2) Complex shapes created using
Fourier series $\rho(\alpha) = a_0 + \sum_{k=1}^5 a_k \sin(k
\alpha)+b_k \cos(k \alpha)$ in polar coordinates with random
coefficients $(a,b)$ (Fig.~\ref{fig:total_cost}b). Derivatives,
curvature and total cost integral can be computed accurately for
these shapes. We then measure the error relative to the true length
of the curve. This experiment verifies that the approximation makes
sense. We do not claim that the accuracy is comparable with
state-of-the-art techniques of approximation curvature of digital
curves, however such comparison could be informative in the future.
\par
Figure~\ref{fig:total_cost}(a,b) shows a bias of our model to
overestimate the true cost. One of the reasons behind this is the
fact that Manhattan length is larger than Euclidean. While this is
not essential for shape optimization (makes a slightly different
prior), we show that the model actually can compensate to some
extent for this bias. Wa apply Alg.2 to retrain costs $\bc$ of the
class of Fourier shapes. Figures~\ref{fig:total_cost}(c,d),
evaluated on the independent samples, show a reduced bias.
%
\input{tex/fig3.tex}
%
%
\input{tex/fig4.tex}
\input{tex/fig5.tex}
%
%
%
%
\par
{\bf Shape Optimization.}
We start with simpler problems, where part of the true shape is hidden and the task is to find reconstruction with lowest total curvature cost. This is a good test to inspect what is our shape prior. Let $F\subset \V$ be set of pixels restricted to foreground (shape) and $B\subset \V$ pixels restricted to background. Unary term of~\eqref{energy} Are set as flowing
\begin{equation}
\theta_{v}(x_v) = \begin{cases}
\inf, \tab (x_v=0\ \wedge\ v\in F)\ \vee\ (x_v=1\ \wedge\ v\in B)\\
0, \tab \mbox{otherwise}\\
\end{cases}
\end{equation}
So in the region $\V\backslash (F\cup B)$ unaries are always $0$. Fig.~\ref{fig:inpaint_circle} shows example of such inpainting problem. After 2000 TRW-S iterations many tree min-marginals are close to 0, so the discrete labeling obtained from them has artifacts depending on whether it was $+0$ or $-0$. We then construct a restricted problem by considering only pixels and patterns with tree min-marginals below some threshold and solve this restricted problem with primal LP solver. Rounding of the latter gives a more accurate result.
\par
We investigated in more detail the model of~\cite{Schoenemann09}. Its main property is that there is a pre-specified set of quantized directions. We consider restricted scenarios (Fig.~\ref{fig:inpaint_line_1_4}) where it is evident that optimal shape can be described by a path in the graph. We used 16-connected graph. For two consequent edge elements of the boundary we took the approximation to squared curvature as ~\cite[$G_2$]{Bruckstrein07}.
\begin{equation}\label{curv_approx_scho}
A^2\frac{l_1+l_2}{l_1 l_2},
\end{equation}
where $A$ is angle between the line segments and $l_1, l_2$ their lengths. This is similar to~\cite{Schoenemann09} but symmetric. Another (not essential) difference form~\cite{Schoenemann09} is that they construct edge elements by subdividing each pixel whereas we consider edge elements with end points only in integer grid nodes and allow intersections.
\par
We observed that lines at directions which are not in the model (line at $1/4$ slope in Fig.~\eqref{fig:inpaint_line_1_4}a) are poorly approximated by the model. Indeed, the best approximation to the line has many small ``steps'', whereas a minimal boundary in the model makes one large step. We think this effect results in visible artifacts in real segmentation problems.
Fig.~\ref{fig:inpaint_line_1_4}b shows reconstruction of a quarter of circle similar to the circle test we did for our model. Let us also note, that approximation~\eqref{curv_approx_scho} is for small angles and model~\cite{Schoenemann09} could potentially benefit from using a better approximation for large angles.
%
\input{tex/fig6.tex}
%
%Description of inpainting problem, details of experiments.\\
%Simplification of [Schoenemann09] model.\\
%
%
%
%
%
%
\input{tex/fig7.tex}
%
%

%\begin{figure}[tr]
%\begin{center}
%\setlength{\tabcolsep}{2pt}
%\setlength{\doublerulesep}{0pt}
%\setlength{\fboxsep}{0.3pt}
%%\input{}
%%\fbox{
%\begin{tabular}[t]{cc}
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/scho/line_1_4x}}&
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4_task}}\\
%(a) & (b)\\
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4}}&
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4_lp}}\\
% (c) & (d)\\
%%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4}}\\
%%\includegraphics[width=0.5\linewidth,height=0.2\linewidth]{fig/dummy}%
%%\includegraphics[width=0.5\linewidth,height=0.2\linewidth]{fig/dummy}%
%\end{tabular}
%
%\caption{(a) Model of~\cite{Schoenemann09}: optimal solution (black) and thought best line approximation (blue). (b) Similar inpainting problem for our model: interior of the green rectangle is hidden and it to be reconstructed. (c) solution from TRW-S tree min-marginals. (d) Solution of LP-relaxation.
%%(b) Unaries for inpainting problem in our model. (c) LP relaxed solution (d) Rounding of LP.
%}.
%\label{fig:inpaint_line_1_4}
%\end{center}
%\end{figure}
%%
%%
%\begin{figure}[tr]
%\begin{center}
%\setlength{\tabcolsep}{0pt}
%\setlength{\doublerulesep}{0pt}
%%\input{}
%%\fbox{
%\begin{tabular}{c}
%\includegraphics[width=0.5\linewidth]{fig/inpaint/scho/circle_16}%
%%\includegraphics[width=0.5\linewidth]{fig/dummy}%
%\end{tabular}
%\caption{(a) Model of~\cite{Schoenemann09}: optimal solution (black) with boundary conditions representing quarter of a circle (red).% (b) ??.
%}
%\label{fig:schoenemann_circle}
%\end{center}
%\end{figure}
%
%
%
{\bf Real Images.}
Let us have image $I:\V\to \C$, Given color models for foreground $p_{\rm FG}(I_v)$ and backgound $p_{\rm BG}(I_v)$, unary terms are set as
\begin{equation}
\begin{array}{l}
\theta_v(1) = -\log p_{\rm FG}(I_v)\\
\theta_v(0) = -\log p_{\rm BG}(I_v),
\end{array}
\end{equation}
so $\theta_v(0)-\theta_v(1)$ is the log-likelihood for each pixel.
Fig.~\ref{giraffe}a shows exemplar image with seeds of foreground and background. We estimate the color models as Gaussian mixture with 10 components. The log-likelihoods are shown in Fig.~\ref{giraffe}b.

\input{tex/fig8.tex}

{\bf Generic Patterns}

\input{tex/fig9.tex}


==> tex/experiments_old.tex <==
\section{Experiments}\label{experiments}

We begin by a discussion of our learning procedure. Then we discuss various results for inpainting and image segmentation and also show a detailed comparisons with \cite{Schoenemann09}.


%We assume that
% Out into exp section.
%As test shapes we generate parabola with 3 parameters: curvature, orientation and offset from the center. As initial splitting of the training (instead of step 1) data we use uniform division of the parameter space: we assign all shapes within a small range of curvature, orientation and shift to one pattern and perform step 2. A model trained in this way with 16 orientations and 3 curvature intervals performed already quite well in the experiments. However more detailed evaluation showed that approximation could be improved by few iterations of the full algorithm (Fig.~\ref{fig:alg1_progress}).
%
%


{\bf Cost approximation.}
To learn 96 patterns of size $K=8$ we initially, sampled $N=10000$ random quadratic curves in the $K{\times}K$ window passing close to the center: location at $(K/2,K/2)$ is a boundary location, Fig.~ref{fig:pointwise}.
We split them into $32$ orientations and $3$ curvature intervals to learn the initial estimate. Fig.~\ref{fig:alg1_progress} shows the error of the estimate measured by~\eqref{pointwise_approx} and progress of Alg.1., while Fig.~\ref{fig:pointwise} shows individual approximations of the test points.
\par
It is seen from Fig.~\ref{fig:pointwise} that pointwise approximation is not accurate. However, we hope than when the costs are summed up along the boundary they will give a good approximation on average. For this purpose we sampled larger shapes for which we can compute true total cost exactly and compared to our model's total cost. Fig.~\ref{fig:total_cost}(a,b) shows this experiment for two classes of shapes. Circular shapes of size $100{\times}100$, with random radius sampled uniformly in [5 50] and random subpixel shift, Fig.~\ref{fig:total_cost}a. And more difficult  shapes, created using Fourier series $\rho(\alpha) = a_0 + \sum_{k=1}^5 a_k \sin(k \alpha)+b_k \cos(k \alpha)$ in polar coordinates with random coefficients $(a,b)$ , Fig.~\ref{fig:total_cost}b. Derivatives, curvature and total cost integral can be computed accurately for these shapes. We then measure the error relative to the true length of the curve. This experiment verifies that the approximation makes sense. We do not claim that the accuracy is comparable with state-of-the-art techniques of approximation curvature of digital curves, however such comparison could be informative in the future.
\par
Figure~\ref{fig:total_cost}(a,b) shows a bias of our model to overestimate the true cost. One of the reasons, being that Manhattan length is larger than Euclidean. While, this is not essential for shape optimization (makes a slightly different prior), we show that the model actually can compensate to some extend for this bias. Wa apply Alg.2 to retrain costs $\bc$ of the class of Fourier shapes. Figures~\ref{fig:total_cost}(c,d), evaluated on the independent samples, show a reduced bias.
%
\input{tex/fig3.tex}
%
%
\input{tex/fig4.tex}
\input{tex/fig5.tex}
%
%
%
%
\par
{\bf Inpainting Example.}
In inpaiting the goal is to reconstruct an underlying, given shape, while only some parts of the shape are visible to algorithm. 
This is a useful test to inspect our shape prior model. Let $F\subset \V$ be the set of pixels restricted to foreground (shape) and $B\subset \V$ pixels restricted to background. The unary term of~\eqref{energy} are set as follows
\begin{equation}
\theta_{v}(x_v) = \begin{cases}
\inf, \tab (x_v=0\ \wedge\ v\in F)\ \vee\ (x_v=1\ \wedge\ v\in B)\\
0, \tab \mbox{otherwise} \ . \\ 
\end{cases}
\end{equation}
So in the region $\V\backslash (F\cup B)$ the unaries are exactly $0$. Fig.~\ref{fig:inpaint_circle}(a) shows example of an inpainting problem for a circle. The result after 2000 iterations of TRW-S (b) has many tree min-marginals, which are close to 0 (green). Hence the discrete labeling (c) has artifacts depending on whether the min-marginals were $+0$ or $-0$.
We then construct a restricted problem (d) by considering only pixels and patterns where the tree min-marginals are below some threshold and solve this restricted problem with a primal LP solver (e). Rounding of this solution gives a more accurate result (f). It is important to note that the original circle still has a lower energy then this solution.
%
\input{tex/fig6.tex}
%


{\bf Comparison with Schoenemann et al. \cite{Schoenemann09}}
The main property of the model of~\cite{Schoenemann09} is that there is a pre-defined set of quantized directions. 
For comparison, we considered a restricted scenarios (Fig.~\ref{fig:inpaint_line_1_4}) where it is evident that the optimal shape has to be described by a path in the graph. We used a 16-connected graph. For two consequent edge elements, of the boundary, we approximated the squared curvature as
$A^2\frac{l_1+l_2}{l_1 l_2}$, \cite{Bruckstrein07} ($G_2$),
%\begin{equation}\label{curv_approx_scho}
%A^2\frac{l_1+l_2}{l_1 l_2},
%\end{equation}
where $A$ is angle between the line segments and $l_1, l_2$ their lengths. This is similar to~\cite{Schoenemann09} but a symmetric form. Another (not essential) difference of our re-implemtation of~\cite{Schoenemann09} is that they construct edge elements by subdividing each pixel, whereas we model edge elements by end-points in a discrete grid (where edges can also intersect).

Fig.~\ref{fig:inpaint_line_1_4} and  fig.~\ref{fig:inpaint_circle}(f) compare our model with \cite{Schoenemann09}. The main conclusion is that for both examples, a straight line and a circle, our model approximates the true curvature considerably better.  
We observed that lines at directions which are not perfectly modeled in ~\cite{Schoenemann09} (e.g. the line at $1/4$ slope in fig.~\ref{fig:inpaint_line_1_4}a) have a very large approximation error. Indeed, the best approximation to the line in fig.\ref{fig:inpaint_line_1_4}a has many small ``steps'', whereas the optimal boundary in the model of~\cite{Schoenemann09} makes only one large ``step''. We believe that this effect results in visible artifacts in real segmentation problems (see e.g. legs in fig. \ref{giraffe}f).
%Fig.~\ref{fig:inpaint_line_1_4}b shows reconstruction of a quarter of circle similar to the circle test we did for our model. 

%Let us also note that the approximation~\eqref{curv_approx_scho} is for small angles and model~\cite{Schoenemann09} could potentially benefit from using a better approximation for large angles.

%The main conclusion is that our model gives a considerably better approximation of the true curvature for both a straight line, (d) versus (a), and a circle (b) versus fig.\ref{fig:inpaint_circle}(f).  

%
\input{tex/fig7.tex}
%
%

%\begin{figure}[tr]
%\begin{center}
%\setlength{\tabcolsep}{2pt}
%\setlength{\doublerulesep}{0pt}
%\setlength{\fboxsep}{0.3pt}
%%\input{}
%%\fbox{
%\begin{tabular}[t]{cc}
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/scho/line_1_4x}}&
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4_task}}\\
%(a) & (b)\\
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4}}&
%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4_lp}}\\
% (c) & (d)\\
%%\fbox{\includegraphics[width=0.5\linewidth]{fig/inpaint/line_1_4}}\\
%%\includegraphics[width=0.5\linewidth,height=0.2\linewidth]{fig/dummy}%
%%\includegraphics[width=0.5\linewidth,height=0.2\linewidth]{fig/dummy}%
%\end{tabular}
%
%\caption{(a) Model of~\cite{Schoenemann09}: optimal solution (black) and thought best line approximation (blue). (b) Similar inpainting problem for our model: interior of the green rectangle is hidden and it to be reconstructed. (c) solution from TRW-S tree min-marginals. (d) Solution of LP-relaxation.
%%(b) Unaries for inpainting problem in our model. (c) LP relaxed solution (d) Rounding of LP.
%}.
%\label{fig:inpaint_line_1_4}
%\end{center}
%\end{figure}
%%
%%
%\begin{figure}[tr]
%\begin{center}
%\setlength{\tabcolsep}{0pt}
%\setlength{\doublerulesep}{0pt}
%%\input{}
%%\fbox{
%\begin{tabular}{c}
%\includegraphics[width=0.5\linewidth]{fig/inpaint/scho/circle_16}%
%%\includegraphics[width=0.5\linewidth]{fig/dummy}%
%\end{tabular}
%\caption{(a) Model of~\cite{Schoenemann09}: optimal solution (black) with boundary conditions representing quarter of a circle (red).% (b) ??.
%}
%\label{fig:schoenemann_circle}
%\end{center}
%\end{figure}
%
%
%
{\bf Image Segmentation.}
We use a standard model for interactive image segmentation, as defined in \cite{BJ01}. Based on user brush strokes, we compute likelihoods using a standard Gaussian mixture model (GMM) with 10 components.
%Let us have image $I:\V\to \C$, Given color models for foreground $p_{\rm FG}(I_v)$ and background $p_{\rm BG}(I_v)$, unary terms are set as
%\begin{equation}
%\begin{array}{l}
%\theta_v(1) = -\log p_{\rm FG}(I_v)\\
%\theta_v(0) = -\log p_{\rm BG}(I_v),
%\end{array}
%\end{equation}
The unaries define the negative log-likelihood ratio as, $\theta_v(0)-\theta_v(1)$, for each pixel.
A result is shown in fig.~\ref{giraffe}. Note that the curvature prior (e,f) is able to connect the giraffe's legs, compared to a length prior (c). 
The final result of our method (e) and \cite{Schoenemann09}(f) are of similar quality, despite the fact that we use a grid with much coarser resolution.

\input{tex/fig8.tex}

% {\bf Generic Patterns}

% \input{tex/fig9.tex}

==> tex/fig_alg1_progress.tex <==
\begin{figure}[tr]
\begin{center}
\setlength{\tabcolsep}{0pt}
\setlength{\doublerulesep}{0pt}
\includegraphics[width=0.5\linewidth]{fig/pointwise/alg1_progress}%
\caption{Objective of~\eqref{pointwise_approx} during iterations of Alg.1. Red curve is evaluated on training data and green dashed curve is evaluated on the independent test data. There is sufficiently many samples that training error is very close to test error. }
\label{fig_alg1_progress}
\end{center}
\end{figure}

==> tex/fig_giraff_parametric.tex <==
\begin{figure}%[tr]
\begin{center}
\setlength{\figwidth}{0.31\linewidth}
\setlength{\tabcolsep}{2pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0.2pt}
%\input{}
%\fbox{
\scriptsize
\begin{tabular}{ccc}
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_002}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_010}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_020}}\\
2 & 10 & 20\\
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_100}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_500}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_1000}}\\
100 & 500 & $>$1000\\
\end{tabular}
%
%\includegraphics[width = \linewidth, height = \linewidth]{fig/dummy}
%}
\end{center}
\caption{Segmentation with curvature prior (our model). The strength of the prior is below each image. Above a certain strength of the prior (here 1000) the model stops smoothing the shape, because each local $8{\times}8$ window is already maximally smooth according to the model.}
\label{fig_giraff_parametric}
\end{figure}

==> tex/fig_giraff_parametric_BJ.tex <==
\begin{figure}%[tr]
\begin{center}
\setlength{\figwidth}{0.31\linewidth}
\setlength{\tabcolsep}{2pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0.2pt}
%\input{}
%\fbox{
\scriptsize
\begin{tabular}{ccc}
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_001.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_002.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_006.png}}\\
0.15 &   0.3 &    0.9\\
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_007.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_010.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_020.png}}\\
1.0 &    1.5 &    3.0\\
\end{tabular}
%
%\includegraphics[width = \linewidth, height = \linewidth]{fig/dummy}
%}
\end{center}
\caption{Segmentation with length prior (8-connected model) for various strengths of the prior (numbers below each figure).}
\label{fig_giraff_parametric_BJ}
\end{figure}

==> tex/fig_giraff_task1.tex <==
\begin{figure}[tr]
\centering
%
\setlength{\tabcolsep}{5pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0.2pt}
%\input{}
%\fbox{
\begin{tabular}{ccc}
(a)
\begin{tabular}{c}
\fbox{\includegraphics[width=0.2\linewidth]{fig/giraffe/input_t}}
\end{tabular}&
(b)
\begin{tabular}{c}
\fbox{\includegraphics[width=0.2\linewidth]{fig/giraffe/unaries}}
\end{tabular}&
(c)
\begin{tabular}{c}
\fbox{\includegraphics[width=0.2\linewidth]{fig/giraffe/schoenemann-result-16}}
\end{tabular}\\
\end{tabular}
%
%%%%%%%%%%%%%%%
%
%
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cc}
(d)&%
\hspace{-5mm}
\setlength{\figwidth}{0.2\linewidth}
\setlength{\tabcolsep}{1pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0.3pt}
\begin{tabular}{ccc}
\scriptsize
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_001.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_002.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_006.png}}\\
0.15 &   0.3 &    0.9\\
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_007.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_010.png}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_020.png}}\\
1.0 &    1.5 &    3.0\\
\end{tabular}\\
%
%%%%%%%%%%%%%%%%%%%%%
%
(e)&%
\hspace{-5mm}
\setlength{\figwidth}{0.2\linewidth}
\setlength{\tabcolsep}{1pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0.2pt}
\begin{tabular}{ccc}
\scriptsize
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_002}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_010}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_020}}\\
2 & 10 & 20 \\
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_100}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_500}}&
\fbox{\includegraphics[width=\figwidth]{fig/display/giraffe_model12_C3200_I400_icm_1000}}\\
100 & 500 & $>$1000\\
\end{tabular}
%%%%%%%%%%%%%%%%%%%%
\end{tabular}
%
%
\caption{{\bf Image segmentation.}
(a) Image with foreground (green) and background (blue) seeds;
(b) unaries (color coded).
(c) Result copied from \cite{Schoenemann09}.
(d) Segmentation with length prior (8-connected model) for various strength of the prior (numbers below figure).
(e) Segmentation with curvature prior (our model) for various strength of the prior. 
}
\label{fig_giraff_task}
\end{figure}

==> tex/fig_inpaint_circle_lp.tex <==
\begin{figure}[tr]
\begin{center}
\setlength{\figwidth}{0.3\linewidth}
\setlength{\tabcolsep}{2pt}
\setlength{\doublerulesep}{0pt}
\setlength{\fboxsep}{0pt}
%\input{}
%\fbox{
\begin{tabular}{ccc}
\fbox{\includegraphics[width=\figwidth]{fig/inpaint_circle/b_diffuz_reparametrized}}&
\fbox{\includegraphics[width=\figwidth]{fig/inpaint_circle/c_restriction_area}}&
\fbox{\includegraphics[width=\figwidth]{fig/inpaint_circle/d_lp_inpaint}}\\
(a) & (b) & (c)\\[2mm]
%\vspace{2mm}\\
\end{tabular}
%\includegraphics[width=\linewidth]{fig/inpaint/circle_old.png_circle}%
%\includegraphics[width = \linewidth, height = \linewidth]{fig/dummy}
%}
\end{center}
\caption{ {\bf Restricted LP} (a) Tree min-marginals of TRW-S for a circle inpainting problem: a thin line shows the 0-level contour; (b) The restricted shape inpainting problem obtained by thresholding the absolute values of tree min-marginals, the gray color here shows undecided pixels; (c) Relaxed primal solution of the restricted problem (with 0-level contour).}
\label{fig_inpaint_circle_lp}
\end{figure}

==> tex/fig_total_cost.tex <==
\begin{figure}[tr]
\begin{center}
\setlength{\tabcolsep}{0pt}
\setlength{\doublerulesep}{0pt}
%\input{}
%\fbox{
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig/total_cost/eval_circles_minr5}&
\includegraphics[width=0.5\linewidth]{fig/total_cost/eval_fourier}\\
(a) & (b)\\
\end{tabular}
\includegraphics[width=1\linewidth]{fig/sample_circles_inline}\\
\includegraphics[width=1\linewidth]{fig/sample_fourier_inline}\\
(c)
%
%\includegraphics[width = \linewidth, height = \linewidth]{fig/dummy}
%}
\caption{Approximate Total Cost / Length vs. True Total Cost / Length: (a) Circles, (b) Fourier shapes. (c) Examples of discretized shapes respectively (top circular shapes; bottom Fourier shapes.)}
\label{fig_total_cost}
\end{center}
\end{figure}
